Frequency-Dependent Piezoresistive Effect in Top-down Fabricated Gold Nanoresistors

Piezoresistive strain gauges allow for electronic readout of mechanical deformations with high fidelity. As piezoresistive strain gauges are aggressively being scaled down for applications in nanotechnology, it has become critical to investigate their physical attributes at different limits. Here, we describe an experimental approach for studying the piezoresistive gauge factor of a gold thin-film nanoresistor as a function of frequency. The nanoresistor is fabricated lithographically near the anchor of a nanomechanical doubly-clamped beam resonator. As the resonator is driven to resonance in one of its normal modes, the nanoresistor is exposed to frequency-dependent strains of {$\varepsilon \lesssim 10^{-5}$} in the $4-36~\rm MHz$ range. We calibrate the strain using optical interferometry and measure the resistance changes using a radio-frequency mix-down technique. The piezoresistive gauge factor $\gamma$ of our lithographic gold nanoresistors is $\gamma \approx 3.6$ at 4 MHz, in agreement with comparable macroscopic thin metal film resistors in previous works. However, our $\gamma$ values increase monotonically with frequency and reach $\gamma \approx 15$ at 36 MHz. We discuss possible physics that may give rise to this unexpected frequency dependence.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
